EVEN: An Event-Based Framework for Monocular Depth Estimation at Adverse Night Conditions

Accurate depth estimation under adverse night conditions has practical impact and applications, such as on autonomous driving and rescue robots. In this work, we studied monocular depth estimation at night time in which various adverse weather, light, and different road conditions exist, with data captured in both RGB and event modalities. Event camera can better capture intensity changes by virtue of its high dynamic range (HDR), which is particularly suitable to be applied at adverse night conditions in which the amount of light is limited in the scene. Although event data can retain visual perception that conventional RGB camera may fail to capture, the lack of texture and color information of event data hinders its applicability to accurately estimate depth alone. To tackle this problem, we propose an event-vision based framework that integrates low-light enhancement for the RGB source, and exploits the complementary merits of RGB and event data. A dataset that includes paired RGB and event streams, and ground truth depth maps has been constructed. Comprehensive experiments have been conducted, and the impact of different adverse weather combinations on the performance of framework has also been investigated. The results have shown that our proposed framework can better estimate monocular depth at adverse nights than six baselines.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}
\subsection{Performance on Carla-ADC}
We designed sufficient experiments to demonstrate that our framework effectively fuses information from the event camera into depth estimation. From table II, it can be seen that pure events as input has no way to predict satisfactory depth values due to the limited information, while pure RGB input could perform normally. On the basis of RGB input, either low-light enhancement, adding Sober operator, or fusing  events, will improve the accuracy of depth estimation on top of that, and the enhancement performance varies due to the different enhancement methods. And after adding the edge information extracted by the sober operator directly to the image after low-light enhancement, there is a significant decrease in Abs-rel. The edge information effectively complements the possible errors caused by overexposure or wrong enhancement in the low-light enhancement process. A similar conclusion can be drawn from table III. Meanwhile, the final predictions of the two networks regress to a similar interval.

Figure 6 shows the quantitative result of the initial RGB input, prediction of fusion map, and comparison with depth ground truth. The depth map of the EVEN fusion network has a very noticeable improvement in detail at the edges as well as the object in the distance. This also visually evidences the effective fusion of the edge information and HDR features of events into our network

However, the edge information extracted by the Sober operator is generated from computer graphics while not captured by the real sensor. Finally, event fused with low-light enhancement achieves targeted enhancement of edge features and adds more high dynamic range information to get the best predictions. 

\iffalse
\subsection{Performance on MVSEC}
\begin{table}
\centering
\begin{tabular}{l|l|r|r|r} 
\hline
\multirow{\begin{tabular}[c]{@{}l@{}}Input Sequences \\(Trained on day2)\end{tabular}} & Error Metric ↓~     & \multicolumn{3}{l}{~ ~ ~Accuracy Metric ↑}                                           \\ 
\cline{2-5}
                                                                                             & ~ ~ ~ ~Abs          & \multicolumn{1}{l|}{~ ~α1} & \multicolumn{1}{l|}{~ ~α2} & \multicolumn{1}{l}{~ ~α3}  \\ 
\hline
RGB\_Night1                                                                                  & ~ ~ 4.7747          & 0.6724                     & 0.8819                     & 0.9530                     \\ 
\hline
EVEN\_Night1                                                                                 & \textbf{~ ~ 4.3375} & \textbf{0.6729}            & \textbf{0.8858}            & \textbf{0.9606}            \\ 
\hline
RGB\_Night2                                                                                  & ~ ~ 5.1952          & 0.6643                     & 0.8734                     & 0.9414                     \\ 
\hline
EVEN\_Night2                                                                                 & \textbf{~ ~ 4.4671} & \textbf{0.6788}            & \textbf{0.8898}            & \textbf{0.9600}            \\ 
\hline
RGB\_Night3                                                                                  & ~ ~ 4.7022          & 0.6719                     & 0.8988                     & 0.9633                     \\ 
\hline
EVEN\_Night3                                                                                 & \textbf{~ ~ 4.1098} & \textbf{0.6883}            & 0.8939                     & \textbf{0.9716}            \\
\hline
\end{tabular}
\end{table}
\fi
